On the Performance of Mismatched Data Detection in Large MIMO Systems

We investigate the performance of mismatched data detection in large multiple-input multiple-output (MIMO) systems, where the prior distribution of the transmit signal used in the data detector differs from the true prior. To minimize the performance loss caused by this prior mismatch, we include a tuning stage into our recently-proposed large MIMO approximate message passing (LAMA) algorithm, which allows us to develop mismatched LAMA algorithms with optimal as well as sub-optimal tuning. We show that carefully-selected priors often enable simpler and computationally more efficient algorithms compared to LAMA with the true prior while achieving near-optimal performance. A performance analysis of our algorithms for a Gaussian prior and a uniform prior within a hypercube covering the QAM constellation recovers classical and recent results on linear and non-linear MIMO data detection, respectively.

==> macros/delta_star.tex <==
% This file was created by matlab2tikz v0.4.7 running on MATLAB 8.1.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
\begin{tikzpicture}

\begin{axis}[%
width=5.16317052165354in,
height=3.59478807824803in,
scale only axis,
xmin=0.5,
xmax=1,
xlabel={$\sigma{}^\text{2}$},
xmajorgrids,
ymin=-0.1,
ymax=0.02,
ylabel={$\text{MSE }\Psi\text{(}\sigma{}^\text{2}\text{,}\delta\text{)}$},
ymajorgrids,
legend style={draw=black,fill=white,legend cell align=left},
scaled y ticks = false,
y tick label style={/pgf/number format/.cd, fixed, fixed zerofill,precision=2}
]
\addplot [color=blue,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.00847186823552865\\
0.51	-0.00601453905159377\\
0.52	-0.00370544732742462\\
0.53	-0.00154476341156906\\
0.54	0.000467627376738888\\
0.55	0.00233209087222286\\
0.56	0.00404921374335487\\
0.57	0.0056197763556024\\
0.58	0.0070447284855838\\
0.59	0.00832516758867108\\
0.6	0.00946231935404707\\
0.61	0.010457520309356\\
0.62	0.0113122022622594\\
0.63	0.0120278783886857\\
0.64	0.0126061307976336\\
0.65	0.0130485994203295\\
0.66	0.0133569720875105\\
0.67	0.0135329756729161\\
0.68	0.0135783681937844\\
0.69	0.0134949317705579\\
0.7	0.0132844663581388\\
0.71	0.0129487841701174\\
0.72	0.0124897047255125\\
0.73	0.0119090504547793\\
0.74	0.0112086428083547\\
0.75	0.0103902988167651\\
0.76	0.00945582805653367\\
0.77	0.0084070299807415\\
0.78	0.00724569157726995\\
0.79	0.00597358532146186\\
0.8	0.0045924673932799\\
0.81	0.003104076132037\\
0.82	0.00151013070445061\\
0.83	-0.000187670035805887\\
0.84	-0.00198764851672595\\
0.85	-0.0038881492624897\\
0.86	-0.00588753956984844\\
0.87	-0.00798421006078442\\
0.88	-0.0101765751244192\\
0.89	-0.0124630732598896\\
0.9	-0.0148421673307546\\
0.91	-0.0173123447404596\\
0.92	-0.0198721175374564\\
0.93	-0.0225200224577413\\
0.94	-0.0252546209118061\\
0.95	-0.0280744989223199\\
0.96	-0.0309782670182411\\
0.97	-0.0339645600904978\\
0.98	-0.037032037213876\\
0.99	-0.0401793814392991\\
1	-0.0434052995602611\\
};
\addlegendentry{$\delta\text{=0.48}$};

\addplot [color=black!50!green,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0187120376472885\\
0.51	-0.0165142361546856\\
0.52	-0.0144615838414366\\
0.53	-0.0125542475071614\\
0.54	-0.0107921148602765\\
0.55	-0.00917482768761513\\
0.56	-0.00770181154296512\\
0.57	-0.00637230231847263\\
0.58	-0.00518537002453257\\
0.59	-0.00413994006942631\\
0.6	-0.00323481229916234\\
0.61	-0.00246867803042228\\
0.62	-0.00184013528487104\\
0.63	-0.00134770241107862\\
0.64	-0.00098983026065036\\
0.65	-0.000764913067593964\\
0.66	-0.000671298164312661\\
0.67	-0.000707294653602974\\
0.68	-0.000871181143586086\\
0.69	-0.00116121264132862\\
0.7	-0.0015756266909891\\
0.71	-0.00211264883342677\\
0.72	-0.00277049745626901\\
0.73	-0.0035473880963619\\
0.74	-0.00444153725015284\\
0.75	-0.00545116574191751\\
0.76	-0.00657450169464413\\
0.77	-0.00780978314385727\\
0.78	-0.00915526033058989\\
0.79	-0.0106091977060686\\
0.8	-0.0121698756774135\\
0.81	-0.0138355921207137\\
0.82	-0.0156046636852255\\
0.83	-0.01747542691006\\
0.84	-0.0194462391726276\\
0.85	-0.0215154794861878\\
0.86	-0.0236815491621433\\
0.87	-0.0259428723511849\\
0.88	-0.0282978964759938\\
0.89	-0.0307450925669753\\
0.9	-0.0332829555113638\\
0.91	-0.0359100042250333\\
0.92	-0.0386247817554261\\
0.93	-0.0414258553232051\\
0.94	-0.0443118163094768\\
0.95	-0.0472812801947716\\
0.96	-0.050332886455361\\
0.97	-0.0534652984219457\\
0.98	-0.0566772031052537\\
0.99	-0.0599673109926471\\
1	-0.0633343558194223\\
};
\addlegendentry{$\delta\text{=0.49}$};

\addplot [color=red,solid,line width=2.0pt]
  table[row sep=crcr]{0.5	-0.0285342409606091\\
0.51	-0.0265853741923451\\
0.52	-0.0247786943752848\\
0.53	-0.0231143649049744\\
0.54	-0.0215922757814954\\
0.55	-0.0202120761021536\\
0.56	-0.0189732031441291\\
0.57	-0.0178749083936059\\
0.58	-0.0169162808403585\\
0.59	-0.0160962678231115\\
0.6	-0.015413693680812\\
0.61	-0.0148672764379647\\
0.62	-0.0144556427280369\\
0.63	-0.0141773411373831\\
0.64	-0.0140308541328821\\
0.65	-0.0140146087192757\\
0.66	-0.0141269859568777\\
0.67	-0.0143663294565907\\
0.68	-0.0147309529569823\\
0.69	-0.0152191470772199\\
0.7	-0.0158291853299485\\
0.71	-0.0165593294694794\\
0.72	-0.0174078342428757\\
0.73	-0.0183729516045994\\
0.74	-0.0194529344491293\\
0.75	-0.0206460399104498\\
0.76	-0.0219505322723045\\
0.77	-0.0233646855286765\\
0.78	-0.0248867856299656\\
0.79	-0.0265151324467612\\
0.8	-0.0282480414799152\\
0.81	-0.03008384534274\\
0.82	-0.0320208950385883\\
0.83	-0.0340575610547527\\
0.84	-0.0361922342915535\\
0.85	-0.0384233268436126\\
0.86	-0.0407492726486302\\
0.87	-0.0431685280174872\\
0.88	-0.0456795720581163\\
0.89	-0.0482809070043839\\
0.9	-0.0509710584601116\\
0.91	-0.0537485755673797\\
0.92	-0.0566120311073562\\
0.93	-0.0595600215410989\\
0.94	-0.0625911669970385\\
0.95	-0.0657041112112049\\
0.96	-0.0688975214256599\\
0.97	-0.0721700882500693\\
0.98	-0.0755205254908607\\
0.99	-0.0789475699519808\\
1	-0.0824499812108627\\
};
\addlegendentry{$\delta\text{=0.50}$};

\end{axis}
\end{tikzpicture}%
